Box Supervised Video Segmentation Proposal Network

Video Object Segmentation (VOS) has been targeted by various fully-supervised and self-supervised approaches. While fully-supervised methods demonstrate excellent results, self-supervised ones, which do not use pixel-level ground truth, attract much attention. However, self-supervised approaches pose a significant performance gap. Box-level annotations provide a balanced compromise between labeling effort and result quality for image segmentation but have not been exploited for the video domain. In this work, we propose a box-supervised video object segmentation proposal network, which takes advantage of intrinsic video properties. Our method incorporates object motion in the following way: first, motion is computed using a bidirectional temporal difference and a novel bounding box-guided motion compensation. Second, we introduce a novel motion-aware affinity loss that encourages the network to predict positive pixel pairs if they share similar motion and color. The proposed method outperforms the state-of-the-art self-supervised benchmark by 16.4% and 6.9% $\mathcal{J}$ &$\mathcal{F}$ score and the majority of fully supervised methods on the DAVIS and Youtube-VOS dataset without imposing network architectural specifications. We provide extensive tests and ablations on the datasets, demonstrating the robustness of our method.

==> Master's Thesis Report/01-Introduction.tex <==
\chapter{Introduction}

Video Object Segmentation (VOS) separates objects from their surroundings, segments, and connects them throughout a video sequence. It is a challenging problem as the objects in a video change their appearance due to exposure, rotation, and occlusion. VOS has been solved in two ways, first fully supervised VOS frameworks\cite{Xie, stm, cfbi}, that utilize rich frame-wise manual annotation. Second, self-supervised VOS \cite{vid_col, CorrFlow, Lai}, in contrast to the fully-supervised approach, they do not need annotations. Instead, they explore intrinsic video properties like motion, optical flow, or other representations. Self-supervised VOS provides an impressive approach that avoids the need for expensive frame-wise object masks. However, they suffer from a large performance gap compared to their supervised counterparts.

To the best of our knowledge, we are the first to propose a box-supervised simple VOS method without using any ground truth mask annotation. The central idea of this work is to distinguish similar regions based on motion and color similarity utilizing our novel motion aware affinity loss. Hence, we propose two new components for the affinity loss: first, train time motion generation using a bounding box guided motion compensation method. Second, we propose generating pseudo masks, i.e., an approximation of the ground truth masks as in figure \ref{fig:intro}, derived from the combined color and motion. Our method can be easily integrated into any existing segmentation network by applying the proposed components without modifying the network itself. %We achieve competitive performance compared to supervised baselines and significantly outperform other self-supervised approaches.  
We achieve competitive performance compared to supervised baselines and significantly outperform self-supervised approaches on the established DAVIS benchmark.  

In weakly supervised image instance segmentation bounding box supervision\cite{Tian2020, Lan2021} improves the quality of pseudo mask generation compared to class label supervision\cite{Xploiting2021} with a slight increase in annotation effort. It inspired us to use weak bounding box-based supervision for VOS instead of expensive pixel-wise mask annotations. However, in a video, an object may undergo several transformations like occlusion and camouflage effects, making visual tracking difficult \cite{YangGrouping, Lamdouar}. Consequently, separating the foreground object from the background in a video using only color information can result in sub-optimal performance. However, in contrast to color, object motion in a video is an independent yet complimentary feature that can help to distinguish the object from the background.

We introduce a novel motion calculation pipeline that exploits weak bounding box supervision.  Due to global camera movement, motion computation in a video is inherently noisy. To mitigate this effect, an affine transformation is employed on the current frame, which aligns the backgrounds of subsequent frames. Moreover, the pixels outside the bounding box are exploited for better background characteristics and transformation matrix computation. The improved alignment ensures that the foreground and moving objects are the primary sources of motion response. 

\begin{figure}[tbh]
\begin{center}
  \includegraphics[width=\linewidth]{img/fig-1_5.png}
\end{center}
    \caption{The pair-wise affinity maps are generated based on the frame's color and motion separately. Then, the intersection affinity map(pseudo mask) is created where pixel pairs share similar motion and color characteristics. The intersection improves performance by reducing background noise and generating a sparse, high-precision pseudo mask.}
\label{fig:intro}
\end{figure}

The generated motion is then fused with color to create the pseudo mask for the supervision. The proposed motion aware affinity loss computes the mask-label for an object located inside a box if both motion and color characteristics are similar to their surroundings. It leads to a tight and precise mask computation for a perspective foreground object. For example, Figure \ref{fig:intro} depicts a panda sitting in a bamboo field, where its facial fur has a similar color compared to the wooden background stem. It poses a significant challenge to only distinguish the object pixel from the background based on color similarity\cite{Lamdouar}. Hence, resulting in erroneous mask computations, which include background pixels. However, the inclusion of motion could alleviate this problem, as the motion of an object is invariant to its color. We compute the intersection of pixels with color and motion similarity to get a tight mask around the object. Thus, we hypothesize, it will increase the probability of getting high-quality foreground pixels, which is helpful for network supervision. 



Furthermore, incorporating our novel motion-aware affinity loss requires no architectural changes. Our work's contribution can be summarized as follows:
\begin{itemize}
    \item We are the first to propose a VOS method that employs weak bounding box supervision. Our method is compatible with any existing segmentation framework and does not require any changes to its parameters.    
    \item An improved motion compensation technique is proposed that effectively utilizes the available bounding box coordinates for reducing global camera movement.
    \item A novel motion aware affinity loss is introduced for frame-wise VOS with a pseudo mask generated from pair-wise color and motion similarity.  
    \item We have conducted extensive experiments on multiple datasets and ablation studies. Our method achieved an absolute 7\% $\mathcal{J} \& \mathcal{F}$ improvement on the DAVIS dataset.
\end{itemize}

% Object segmentation is a crucial computer vision task for scene understanding. The current trend to tackle this task is to create thousands of per-pixel annotated frames to train deep neural networks in a fully supervised manner. The time and human cost of this task are enormous. To carry out this task every time for a new use case makes it difficult to pursue despite its accuracy. Bounding boxes are easier to annotate and they act as a prior for the objects inside. But the bounding box can not determine objects accurately which are not axis aligned. So the applications where accurate shape and position of objects are important, per-pixel segmentation is needed. Modern deep learning-based approaches require a huge amount of annotated data in the fully supervised setup. To reduce the annotation task, we intend to use motion calculated using consecutive frames of video data. In this work, we want to leverage a motion map with a bounding box as weak supervision to generate a per-pixel segmentation mask.  \par

% Ideally, the foreground objects should have a higher motion response than the background which acts as a before the shape and location of moving objects. These motion responses are not pixel-perfect. They can come from parts of the object or can overestimate the area. So we should consider the motion map as an approximation of the original ground truth segmentation treated like sparse labels. With these automatically generated sparse annotations, we intend to figure out the pixel-wise segmentation mask or dense annotations. Achieving so would reduce the annotation effort by a large margin, enabling segmentation tasks in application areas where video data is readily available. From video data, our novel motion calculation method can extract motion maps in an offline fashion and train the network with the derived motion definitions.
% The only annotation effort that would be required would be to create the bounding boxes. \par





==> Master's Thesis Report/02-related_work.tex <==
\chapter{Related Work}


\section{Box Supervised Image Instance Segmentation} 
An image instance segmentation network can be trained without a segmentation mask in four ways, key-points\cite{keypoint1,keyscribble}, scribbles\cite{keyscribble,scribble1}, class labels\cite{AhnDGIST,imgtag1,imgtag2,imgtag3,imgtag4}, and bounding boxes\cite{Xploiting2021,Lee,Song2019,Kulharia2020,Hsu2019,Lempitsky2009,Khoreva2017,Rajchl2017,Oh}. The main challenge of box supervision is generating pseudo masks to train the neural network. Existing methods accomplish this using either classical cut-based methods \cite{Kulharia2020, Khoreva2017} or by leveraging neural network activation maps \cite{class_sup}. Among these, the state-of-the-art box supervised instance segmentation methods are BoxInst\cite{Tian2020} and DiscoBox\cite{Lan2021}. BoxInst uses the color of nearby pixels to cluster them and forces the neural network to predict a similar class for the pixels. The pairwise loss and projection loss aid the network in learning segmentation in a weakly supervised manner. DiscoBox, on the other hand, generates pseudo labels through multi-instance learning\cite{Hsu2019}. However, DiscoBox is based on semantic correspondence, which requires multiple views of the same object for training. They complete the task by storing objects from each class in a memory bank. BoxInst and DiscoBox are on par with varying results depending on the backbone used. However, DiscoBox is not directly applicable to VOS because it requires class-level labels to train the correspondence matching. This paper explores box supervision on video data which allows our model to exploit inter-frame dependency for VOS.
% This paper explores the box supervision with multiple video causes to model inter-frame dependency for VOS. 

\section{Segmentation using motion}
Existing works utilize optical flow to approximate the motion of objects. For example, FlowIRN\cite{Liu} uses class activation maps \cite{irn} and dense optical flow\cite{ddflow} to generate pseudo supervision. In Motion Grouping \cite{YangGrouping}, dense optical flow\cite{raft,pwcnet} is used to cluster pixels into the foreground and background. In Deep Fusion\cite{Ellenfeld}, a motion map calculated from sparse optical flow\cite{kanade} is used as network input. Dense optical flow\cite{pwcnet} is used to detect camouflaged animals in\cite{Lamdouar}. The optical flow or its implied motion map is used as input in the mentioned works. In contrast, our work investigates the possibility of training the segmentation network using motion only during training time and generating pseudo labels by fusing it with the color of objects.

\section{Motion Calculation}
Motion from videos is generally calculated with either sparse or dense optical flow and in the case of moving camera global camera motion is reduced before the motion map is generated. For example, some methods\cite{Makino2017MovingobjectDM, Kurnianggoro2016, Huang, Yu2019} use the motion compensation technique to alleviate the camera movement. Background subtraction is used in Deep Fusion~\cite{Ellenfeld} to calculate the motion map. Forward-backward sparse optical flow\cite{Wan2014} is used to further reduce the noise incurred during background modeling. Instead of using only two consecutive frames, some methods\cite{Zhang2012,Xiao2010,Sommer2016,Pollard2012,Chen2012} utilize three frames. Deep neural network-based methods\cite{raft, Jaegle} achieve state-of-the-art performance for predicting dense optical flow with higher inference time. Sparse\cite{bouguet2001pyramidal} or non deep neural network-based dense\cite{Farneback} optical flow is otherwise used to model the background of consecutive frames.

\section{Semi-Supervised VOS} Semi-Supervised VOS is a recent challenge introduced by DAVIS\cite{davis17} and adopted by Youtube-VOS\cite{yvos2018}. The term "semi-supervised" does not refer to the level of supervision used during training. Instead, it only refers to the availability of annotation masks for the first frames of test videos. The challenge is to generate segmentation in the subsequent frames for only the objects given in the first frame. Some methods\cite{Xie, stm, cfbi, afburr, feelvos, gc, osvos-s, siammask, osvos, osmn, msk, rgmp, onavos, rvos, s2s, premvos} solve the task in a fully-supervised setup, where segmentation masks are used as supervision during training. Others trained their models in a self-supervised way\cite{vid_col, CorrFlow, Lai, cycletime, uvc, rpmnet, lu2020learning}, some of which exploit deep optical flow to generate segmentation. Self-supervised methods perform worse compared to the fully supervised setup. We use bounding box annotations to supervise the segmentation network.



% \begin{itemize}
%     \item General Introduction
%     \item Classical Approaches
%     \item Big Data Processing
%     \item ML based 
%     \item RL based 
% \end{itemize}

% Highlight the usefulness, advantages and disadvantages of each technology.

% In this chapter, we talk in brief about some of the existing methods that have been adopted to the objective of weakly supervised segmentation, highlighting their approach, performance and limitations or trade-offs with respect to the objective.


% \section{Weakly Supervised Object Segmentation}

% \subsection{Motion generation}
% \subsection{Motion Compensation}
% \subsection{Motion Calculation}
% \subsection{Motion Clustering}

% \section{Data-set}

% \section{Network Architecture}

% \section{Affinity loss}

% \section{Miscellaneous}






==> Master's Thesis Report/03-Data.tex <==
\chapter{Data}

\section{YouTube-VOS Data-set Description}
YouTube Video Object Segmentation data-set has per frame annotations only in the training set. In validation and test set, it has only first frame annotation mask and no categorical information. These can only be validated in the their server which includes segmentation, detection and tracking of objects all together. The goal of this thesis is not to track object throughout videos. The goal is to exploit motion calculation of which requires previous and next frame. So we have split the train data into train, valid and test set in a 80:10:10 ratio. Further we have got rid of some still objects, for example, bucket, sign, toilet in one of our ablation studies to see the actual effect of our method on moving objects only. We have tested previous works on this modified data-set for comparability.

\section{Data set Preparation}

\subsection{Data-set Split}
Split Youtube-VOS 2019 Train into train-train: train-val: train-test = 80:10:10
(2730, 426, 315, 3471)
\subsection{Balancing Classes}

\subsection{Removing Classes}



\subsection{Original and derived data-set in numbers}



==> Master's Thesis Report/04-techniques.tex <==
\chapter{Methods}


\label{sec:method}
We first introduce our novel motion compensation and generation pipeline, section \ref{sec:motion_calc}, and the motion aware affinity loss, in section \ref{sec:loss}.
The segmentation network and object tracker used in this paper are explained in section \ref{sec:network}.

\section{Compensating Global Camera Motion}
If we can align the background of previous frame to current frame, we remove the camera motion. The only motion remains should come from moving objects. The basic steps in Fig. \ref{fig:as} are given below.

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]{img/remove_motion.png}
\caption{Global Camera Motion removal.}
\label{fig:as}
\end{figure}

\begin{enumerate}
    \item Sample background points from previous frame
    \item Detect corresponding points in current frame with sparse optical flow
    \item Calculate affine transformation matrix from these pair of points.
    \item Apply the transformation to the whole previous frame
    \item Apply frame difference.
\end{enumerate}







\section{Proposed Motion Calculation Pipeline}
\label{sec:motion_calc}
Unlike in an image, the movement of an object can be assessed in the video. In addition to the object's motion, a moving camera can add apparent movement to a video because of the shifting point of view. In the presence of this global camera motion, the computation of motion maps is an intricate task and subject to ongoing research  \cite{Makino2017MovingobjectDM, Kurnianggoro2016, Huang, Yu2019}. Figure \ref{fig:pipeline}, depicts our novel motion computation pipeline that mitigates the earlier effect through refinement of motion using multiple filters and given bounding boxes. 

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{img/full_motion_pipeline_2.png}
\caption{\textbf{Proposed motion calculation pipeline.} The first step, is box-guided motion compensation to reduce camera movement. At second, the motion maps from the previous to the current frame ( $M'_{t-1}$) and from the current to the next frame ($M'_{t+1}$) are derived by the two-frame difference method. Finally, we combine $M^{'}_{t-1}$ and $M^{'}_{t+1}$ (three-frame difference) to generate superior motion map ($\mathcal{M}_t$) for current frame ($F_t$).}
\label{fig:pipeline}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{img/motion_compensation2.png}
    \caption{Improvement of motion map with additional filters.}
    \label{fig:compensation_example}
\end{figure}

\subsection{Box Guided Motion Compensation:} 
In the case of a stationary camera, motion can be calculated by background subtraction~\cite{Ellenfeld} from consecutive frames. However, in a video captured with a moving camera, the background moves as well. In order to reduce background motion the previous and current frames must be co-registered, i.e., the backgrounds of those frames must be aligned. This is known as motion compensation\cite{1997, hartley_zisserman_2004}. 
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{img/compensation2.png}
    \caption{A set of feature points $\{A,B\} \subseteq \mathcal{F}$ are extracted from the previous frame $F_{t-1}$ that lies in region outside the box. 
    Let $\{A^{'}$,$B^{'}\}$ is the forward projection of $\{A,B\}$ and $\{A^{''}$,$B^{''}\}$ is backward projection of $\{A^{'}$,$B^{'}\}$ obtained from sparse optical flow. Finally, we took the point that represents better background properties or if the original point has less distance from its reverse projected point, in the example its $(B, B^{''})$.}
    \label{fig:compensation}
\end{figure}
%Let, a
At time $t$ the previous frame $F_{t-1}$ is aligned to the current frame $F_t$ with a homography matrix $\mathcal{H}$. The homography matrix $\mathcal{H}$ is the affine transformation between the point pairs from $F_{t-1}$ and $F_t$. $\mathcal{H}$ can be calculated by sampling feature points from $F_{t-1}$ and $F_t$ which are matched with the RANSAC-algorithm\cite{ransac}.
We use \cite{323794} for extracting feature points. Notably, this co-registration works well if these feature points come from the background, not from the foreground. Hence, bounding boxes can be exploited in a weakly supervised setup to sample feature points only from outside the box (Box Filter (BF)). However, annotations usually only comprise primary objects, not all the moving instances in the video. For further refinement of the feature points and a better background modeling, a forward-backward sparse optical flow \cite{Wan2014} (using Forward-Backward Filter (FBF)) is employed. Figure \ref{fig:compensation}, depicts our forward ($\{A^{'}$, $B^{'}\}$) and backward ($\{A^{''}$, $B^{''}\}$) projection of points from original A and B. Finally, we remove points which have an L2 distance $D_A$ between the original point (i.e., A) and backward projected point (i.e.,$A^{''}$) greater than $\tau$ with

\begin{equation}
\label{eq:boxmotion}
    \tau = median(\{D_P|P \in \text{feature points}\}).
\end{equation}

Resulting points derived from Eq. \ref{eq:boxmotion} increases the probability of better background modeling.  Hence, the homography matrix $\mathcal{H}$, obtained from these remaining points are used to transform $F_{t-1}$ to the co-registered frame $A_{t-1}$ as shown in Figure \ref{fig:pipeline}. Finally, the motion from \textbf{two frame difference} is obtained as $M'_{t-1} = |F_t-A_{t-1}|$ corresponds to a background subtraction. Figure \ref{fig:compensation_example} shows the improvement of the motion map for the moving objects with the proposed feature point filtering.  

% The indiscriminate movement of primary video instances is problematic and it is burdensome for the two-frame difference due to its short temporal span. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{img/three_frame_example3.png}
    \caption{Examples of improved motion map with 3-frame difference.}

    \label{fig:three_frame}
\end{figure}

\subsection{Three Frame Difference:} Often, indiscriminate movement between two consecutive frames causes low quality motion maps due to the short temporal span. For example, the fast-moving bike in Figure \ref{fig:three_frame}A, seems to appear twice. Whereas, in Figure \ref{fig:three_frame}D, the horse leg has thick edges due to its slow movement. 

To alleviate these problems, a longer temporal difference or three-frame difference has been proposed \cite{Zhang2012,Xiao2010,Sommer2016,Pollard2012,Chen2012}.    
Here, the next frame motion map ($M^{'}_{t+1}$) from $F_t$ to $F_{t+1}$ is computed similarly to the two-frame difference. Finally, the motion map $\mathcal{M}_t$ with three-frame difference is obtained as



\begin{equation}
\mathcal{M}_t=\left\{\begin{array}{cc}
M^{'}_{t-1} & \text { if } M^{'}_{t-1} - M^{'}_{t+1} <\tau_2 \\
0, & \text { else }
\end{array}\right.
\label{eqn:three_frame_diff}
\end{equation}
where $\tau_2$ is a predefined threshold. Here the motion response of a certain pixel in $M^{'}_{t-1}$ is filtered out to zero if it is greater than that of $M^{'}_{t+1}$ up to the threshold $\tau_2$. 

\section{Pseudo Mask Generation}
\label{sec:loss}
The generated motion is combined with color to create a pseudo mask that approximates the ground truth mask. However, the generated pseudo mask is inherently noisy because of impurities in motion. Thus, penalizing the network with global pixel-wise cross-entropy loss would be erroneous. Instead, we can classify pairs of pixels in close vicinity by looking at their color and motion. The idea is to define pixel pairs as positive, i.e., they belong to the same class if they share similar colors and motion in a local neighborhood. Finally, an affinity loss\cite{Wu, Ke2018} is employed to assign the same class for each positive pixel-pair if they share a similar pair-wise affinity. We impose only positive affinity loss, which means that only mispredicted positive pairs from the segmentation network will contribute to the overall loss.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{img/affinity_map6.png}
    \caption{An illustrative example of the motion aware affinity loss in a 3x3 pixel grid of an image. In Fig. A and B pixels with a similar color/motion are indicated by the same color. Fig. C combines the color(left) and motion(right) properties from Fig. A and B. Fig. D shows the final affinity map. Groups of pixels with the same color/motion properties are marked by the white boundary ( e.g., $\{A,E,H\}$, $\{B,F,I\}$). With pairwise pixel matching, each of these groups gets clustered into the same class during training.}
    \label{fig:intersect_aff_map}
\end{figure}



Suppose we are given an Image I, and we are computing the proposed affinity loss on a $3\times3$ image patch as depicted in Figure \ref{fig:intersect_aff_map}. Consider pixels $A$ and $B$ and their corresponding motion values are $\mathcal{M_{A}}$ and $\mathcal{M_{B}}$ and  $\mathcal{C_{A}}$ and $\mathcal{C_{B}}$ are their color values. The motion and color similarities (the higher the value the more similar it is)  between these pixels are $\mathcal{\psi_{A,B}} \in \, ]0,1]$, and $\mathcal{\phi_{A,B}}\in \, ]0,1]$. These similarities can be expressed as 


\begin{equation}
    \begin{aligned}
        \mathcal{\psi_{A,B}} = exp(-\|\mathcal{M_{A} - M_{B}\| * \eta})\\
        \mathcal{\phi_{A,B}} = exp(-\|\mathcal{C_{A} - C_{B}\| * \eta})
    \end{aligned}
    \label{eq:sim}
\end{equation}

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{img/mg.png}
    \caption{Pseudo mask generation process. First intermediate masks are generated from RGB frames and motions which are then combined into the Pseudo Mask.}
    \label{fig:intersect_aff_map}
\end{figure}

where $\eta$ is a hyper-parameter. We hypothesize that two pixels with similar color or motion are likely to be in the same class. For example, the pixel pair $(A, E)$ in Figure \ref{fig:intersect_aff_map}, has similar color and motion, indicating that both pixels belong to the same class. The pixel pair $(A, B)$, on the other hand, has a high color similarity but a low motion similarity, so they should be classified into different classes. Finally, for a pair of pixels their motion ($\Psi_\mathcal{A, B}$) and color ($\Phi_\mathcal{A, B}$) affinity, based on the similarity threshold, can be defined as 

\begin{equation}
    \begin{aligned}
        \begin{array}{cc}
        \Psi_\mathcal{A,B}=
        \left\{ \begin{array}{ll}
            1 &\mathcal{\psi_{A,B}} > \tau_m\ \\
            0 &\text{else}
        \end{array} \right. ,&
        \Phi_\mathcal{A,B}=
        \left\{ \begin{array}{ll}
            1 &\mathcal{\phi_{A,B}} > \tau_c\ \\
            0 &\text{else}
        \end{array} \right.
        \end{array}
        \end{aligned}
        \label{eq:aff_mc}
    \end{equation}

 where $\tau_m $ and $\tau_c$ are the motion and color similarity threshold. 
 The proposed loss is calculated only for pixel-pairs with high similarity, i.e., positive affinity. It essentially means the network is trained to predict segmentation with the correct pixel pairs. Hence, constructing high precision positive pixel pairs from motion and color information can significantly boost the network performance. Thus, an affinity ($\mathcal{I_{A,B}}$) between two pixel $(A,B)$ can be defined as  
 \begin{equation}
    \mathcal{I_{A,B}} = \Psi_\mathcal{A,B} \cap \Phi_\mathcal{A,B}.
    \label{eq:aff_i}
\end{equation}
An intersecting subset-based affinity (Eq. \ref{eq:aff_i}) effectively reduces the noise from each set. A more detailed experiment and discussion on the selection of combined motion and color-based affinity can be found in Table \ref{tab:ablation_fusion}.





\section{Motion Aware Affinity Loss}
Pairwise Affinity has long been used for video segmentation in various way like using ground truth label\cite{Wu,Ke2018,Zhang}, color\cite{Tian2020}, class activation map\cite{AhnDGIST}, gradient of optical flow\cite{Liu}, or geodesic distances or radius\cite{Sumengen2006}. We use motion and color characteristic of objects to formulate an affinity loss.

Let the confidence score of the segmentation network for pixels $A$ and $B$ being foreground be $\rho_{\mathcal{A}}$ and $\rho_{\mathcal{B}}$. Then the confidence of these two pixels being predicted as the same class(either foreground or background) is $\rho_{\mathcal{A,B}}$, and computed as 

\begin{equation}
    \rho_{\mathcal{A,B}}= \rho_\mathcal{A} * \rho_\mathcal{B} + (1-\rho_\mathcal{A}) * (1-\rho_\mathcal{B}),
    \label{eq:same_class}
\end{equation}
 where the confidence of the pixel pair being foreground is $\rho_\mathcal{A} * \rho_\mathcal{B}$, or being background is  $(1-\rho_\mathcal{A}) * (1-\rho_\mathcal{B})$. Let $\mathcal{P}$ be the set of pixel pairs where at least one pixel falls inside the bounding box. For a pixel pair A and B, our motion aware affinity loss, $\mathcal{L_{A,B}}$ , is calculated as 

\begin{equation}
    \mathcal{L_{A,B}} = -\mathcal{I_{A,B}} * log(\rho_{\mathcal{A,B}}).
    \label{eq:pair_loss}
\end{equation}

Finally, for all pairs of pixels in $\mathcal{P}$ we calculate the loss as 

\begin{equation}
    \mathcal{L_{\textit{affinity}}} = \sum_{\mathcal{A,B} \in \mathcal{P}}  \mathcal{L_{A,B}}.
    \label{eq:all_loss}
\end{equation}


\pagebreak

\section{Segmentation Architecture} 
\label{sec:network}
\subsubsection{Proposal Generation}
CondInst\cite{tian2020conditional} has been used as our default segmentation network. It is a Region-Of-Interest(RoI) proposal free segmentation network with fewer parameters and faster computation. Hence, we choose CondInst as our default architecture.  The core of CondInst is built on top of the Feature Pyramid Network (FPN) \cite{lin2017feature} and FCOS \cite{tian2019fcos}. FPN employs multi-scale feature maps for detecting objects from various scales. 
%  Multi-scalar predictions are useful for detecting objects on different scales but can be computationally expensive if done independently. FPN makes the task feasible by sharing computation on multi-scale feature maps. 
FCOS is a proposal-free, anchor-free, fully convolutional one-stage object detector. Instead of assigning multiple anchor boxes\cite{ren2015faster} for each feature point produced from FPN, it predicts only one box. In addition, a center-ness weighting scheme was introduced to filter the boxes far away from the center. Unlike traditional networks \cite{ren2015faster,maskrcnn} that define instances with individual boxes and ROI cropping or pooling, CondInst proposes an instance-aware mask head with conditional convolution. It dynamically generates instance-specific convolutional filter parameters. This conditional convolution learns instance properties without a complicated object detection pipeline. % It extends FCOS loss with an additional mask head loss. 
In this work, the fully supervised mask loss of CondInst is replaced with a projection loss\cite{Tian2020} and the proposed motion aware affinity loss. Projection loss is a specialized 1d intersection-over-union (IoU) loss calculated separately for the height and width of the segmentation mask. The description of each network is briefly discussed below.


\subsubsection{FPN} To detect objects on different scales, multi scalar predictions are useful but can be computationally expensive if done independently from each other. FPN leverages the idea with shared computation on multi scale feature maps with less computation. The feature maps from a standard image backbone are fused in the upsampling phase(top-down pathway) with lateral connections for better activations. Predictions are done on each layer. This can be used as a regional proposal network of Fast-RCNN\cite{fastrcnn}.


\subsubsection{FCOS} This is a proposal free, anchor free, fully convolutional, One stage object detector. Instead of assigning multiple anchor boxes for each pixel in the feature map, it predicts only one box with Left, Right, Top, and Bottom distance from the pixel. To filter far away boxes from the center, a centeredness weighting scheme is developed. When testing, the final score (used for ranking the detected bounding boxes) is computed by multiplying the predicted centeredness with the corresponding classification score. Thus the centeredness can down- weight the scores of bounding boxes far from the center of an object. All the heads share parameters and predict objects at different scales. There are two losses, one for classification which gets weighted by centeredness. The second loss is regression loss for the bounding boxes. Classification loss is normalized by the number of classes and regression loss is normalized by the number of bounding boxes.

 
\subsubsection{CondInst} A fully convolutional network is used to solve instance segmentation, which eliminates the need for ROI cropping and feature alignment. To predict the masks for each instance, CondInst employs instance-aware mask heads. The filters in the mask head change depending on the target instance, which is dynamically generated and conditioned.

CondInst uses instance-sensitive convolution filters as well as relative coordinates appended to the feature maps to take advantage of the location information. It is expected that the network parameters will be able to encode the characteristics of this instance (e.g., relative position, shape, and appearance) and that the network parameters will only turn on the pixels of this instance, avoiding the previously mentioned difficulty.

Mask R-CNN\cite{Hea} represents instances through bounding boxes. CondInst, on the other hand, uses instance-aware filters to represent the instances. To put it another way, CondInst implicitly encodes the instance concept into the mask heads' parameters rather than encoding it into the bounding boxes.

Each location on the FPN's feature maps is associated with an instance, making it either a positive sample or a negative sample, similar to FCOS. The classification head predicts the instance's class based on its location.

The controller's head is used to predict the parameters of the mask head for the instance at the location. This instance's mask is predicted by the mask head. This is the work's primary contribution. To predict the parameters, it concatenates all the parameters of the filters (i.e., weights and biases) together as an N dimensional vector, where N is the total number of the parameters. Because the generated filters contain information about the instance at the location, the mask head with the filters should, in theory, only fire on the pixels of the instance, even if the entire feature map is used as input.

The centeredness and box heads are identical to those found in FCOS. CondInst continues to predict boxes. The predicted boxes are only used in NMS, and there are no ROI operations involved. Furthermore, if mask NMS is used, the box prediction can be removed. This is fundamentally different from previous ROI-based methods, in which box prediction is mandatory.


\section{Tracking}
\label{tracking}
During test-time, the generated proposals are tracked with an optical flow \cite{ilg2017flownet} and an object re-identification \cite{li2017video} network as proposed in PReMVOS\cite{premvos}. In a semi-supervised VOS setting\cite{davis17,yvos2018} ground-truth proposals from the first frame are matched with the next frame proposals using a bipartite matching mechanism. The bipartite matching utilizes a score from IoU overlap wrapped with the optical flow and re-identification score.  The generated proposals for consecutive frames are matched to the previous frame similarly. Some of the proposals from the segmentation network are thus filtered out by the tracker based on IoU overlap.



\section{Incomplete Approaches}
Apart from the method described above, two notable approaches are also explored in this work, which could not achieve the best results. The first one is the self-supervised pre-training of the backbone network, which requires extensive amount of GPU time. The second one is the set based loss formulation, which divides video frames into region clusters based on motion and color properties.


\subsection{Detection focused Contrastive Learning.}
We have used ResNet models pre-trained on Imagenet\cite{imagenet} classification data-set to train the final model. We tried to train the network in a self-supervised fashion as well with contrastive learning framework Barlow Twins\cite{barlow}. In the original paper, Barlow Twins tried to maximize the correspondence between features of two augmented versions of the same image. They minimized the correlation matrix between the set of features retrieved from both augmentations using the same network parameters with an identity matrix of the same dimension. The training required 16 V100 GPUs. 

\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]{img/ssl.png}
\caption{Different augmentations generated to pretrain base network in a self-supervised way with contrastive loss.}
\label{fig:ssl}
\end{figure}

The original method randomly cropped the images to create different views of the same object. We instead use the bounding box coordinates to explicitly encode the object location for one of the augmentations as in Fig. \ref{fig:ssl}. We create three types of multi object-specific crops, e.g, inject background with noise, or blur the background or we simply crop the image with the union of all bounding boxes. One of the three augmentations is selected randomly to match with the original image. The centered object-specific augmentation should force the network to learn only the definition of the object to match with the original image. The resulting backbone weights should encode object-specific properties. This direction did not work out so well because of the scarcity of GPUs. We trained only 25 epochs with 2 RTX-3090 GPUs. The result was worse than the baseline. So the direction was not explored further.




\subsection{Set Loss based on Binned Motion.}
Our objective is to generate supervision of objects that are moving. We have tried to reduce the background motion noise with customized motion compensation and motion calculation techniques. Still, the motion heat map contains background motion noise. Sometimes the noise is quite significant. Our ultimate goal is to group pixels into foreground and background according to their motion values. Up until now, we have been trying to look at a local neighborhood and force the model to classify pixels in that neighborhood as similar if their motion values are similar. We achieved this by sliding a suitable kernel across a spatially reduced heatmap. 


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{img/set_loss.png}
\caption{Pseudo label generation method for set loss.}
\label{fig:set_loss}
\end{figure}


Instead of doing the pixel matching locally, we can try a global approach as well, where we bin pixels inside the bounding box according to their motion values. Keeping in mind that the motion calculation process contains lots of noise, we want to extract sparse foreground and background pixels. We assume that the highest motion pixels should definitely come from objects.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{img/set_loss2.png}
\caption{An example of generated Pseudo label.}
\label{fig:set_loss2}
\end{figure}

Let's assume that we have grouped all the pixels into n different bins according to their motion values. Let the bin with maximum and minimum motion values be $b_{max}$, and $b_{min}$. So we assign all the pixels inside the $b_{max}$ as foreground objects. This gives us confident foreground pixels. We can go further to extract some background pixels as well. 



The bin $b_{min}$ should definitely contain some background pixels. But they could also contain some foreground objects as well. We can either filter out the pixels inside $b_{min}$ that correspond to the most promising colors in $b_{max}$, or we can check if the most promising colors correspond a lot or not between the two bins. If they are similar, we don’t work with $b_{min}$ at all. We can optionally look at the 2nd last bin and so on in that case. In Fig. \ref{fig:set_loss2}, the highest and lowest motion groups are used to extract the foreground and background labels. We applied the proposed affinity loss on this pseudo mask which performed slightly worse. The loss formulation can further be changed to match groups instead of pair of pixels to improve this method. 

% \begin{itemize}
%     \item General Introduction
%     \item Value Iteration ~ parametric and non-parametric approaches.
%     \item Continuous State Space: function approximations. 
%     \item Parametric Approach: RBFs
% \end{itemize}

% Present the Mathematical formulation and algorithm where applicable.

% This chapter talks about some of the general techniques that we have adopted in our project. We explain their functioning and mathematical model, their role with regard to our objective, and modifications that we aim to make in them, if any. 

% \section{Motion Generation}
% \subsection{Motion Compensation}
% \subsection{Motion Calculation}
% \subsection{Motion Clustering}

% \section{Loss Formulation}
% \subsection{Affinity Loss}
% \subsection{Sparse Loss}
% \subsection{Set Based Loss}


% \section{Motion as Input}
% \subsection{Inject Motion Map into backbone}
% \subsection{Inject Similarity Map into backbone}
% \subsection{Injection Method}
% \begin{itemize}
%     \item Simple addition
%     \item One by one Convolution
% \end{itemize}

% \section{Self Supervised Object Representation Learning}
% \begin{itemize}
%     \item Bounding box based weakly supervised five augmentations.
%     \item Backbone to learn Object Detection specific representation in a self supervised way.
%     \item No improvement with less training time.
%     \item Dropped because of sheer amount of GPU needed to train.
% \end{itemize}

% \section{Video Input}
% \subsection{Novel Inter frame communication with object queries}
% Could not connect directly to the thesis topic/ motion.
% \subsection{existing model for comparability}
% Should be the last task if possible.




==> Master's Thesis Report/05-Experiments.tex <==
\chapter{Experiments}

We conduct our experiments on the two most popular video object segmentation datasets, DAVIS-2017\cite{davis17} and Youtube-VOS\cite{Yang2019}. Unless and otherwise specified, we have only used bounding box supervision for training and $\mathcal{J}$\&$\mathcal{F}$ score\cite{davis17} for evaluation throughout our experiments and ablation studies.
We computed the bounding box from the segmentation mask as explicit bounding boxes are not given in both datasets. During test-time, we generate frame-wise proposals and track them throughout the sequence in semi-supervised VOS evaluation settings. As a default baseline network, we employ a state-of-the-art image segmentation network named BoxInst\cite{Tian2020}. It shares a similar CondInst backbone with box-supervised projection and pairwise losses. Our baseline network is trained with only color information. \\
Details of all the hyperparameters can be found in the appendix.

\section{Datasets}
\subsection{DAVIS-2017} DAVIS-2017\cite{davis17} is one of the most widely used VOS datasets where every frame is annotated with a ground truth mask. A predefined training and validation split consists of 60 and 30 videos. \\
\subsection{Youtube-VOS} Youtube-VOS\cite{Yang2019}  was recently proposed as one of the largest video object segmentation datasets. It contains 3,471 training, 507 validation videos with 94 different object categories. Training data contains ground truth mask annotations for every 5th frame while validation contains only for the first frame. 

\subsection{Dataset Preparation}
For training the segmentation network on YoutubeVOS \cite{yvos2018} and DAVIS \cite{davis17} datasets, we first created COCO \cite{coco} style annotations and trained the model with independent frames. We computed the bounding box from the ground truth segmentation mask as no bounding box is available in the datasets. The ground truth mask is not used for any other training purposes. 


\section{Evaluation Metrics}
\subsection{$\mathcal{J}$ \& $\mathcal{F}$ Score } The Jaccard Index $\mathcal{J}$ is the intersection of prediction and ground truth mask over their union. It indicates the region accuracy of the prediction. The contour accuracy $\mathcal{F}$ calculates the f1-score of the boundary pixels with a bipartite matching algorithm. The mean of these $\mathcal{J}$ \& $\mathcal{F}$ is reported as in the DAVIS 2017 \cite{davis17}, for both DAVIS and Youtube-VOS.

\subsection{mAp.} The mean average precision is the area under the precision-recall curve where the IoU threshold determines the positive and negative examples. For initial hyper-parameter tuning, mAp was used as the evaluation metric. We used the implementation from COCO\cite{coco}.



\section{Training Procedure}
We have implemented our method on the detectron2 \cite{wu2019detectron2} or more specifically its adapted version, AdelaiDet \cite{tian2019adelaidet} framework. Our segmentation network is first trained on the YoutubeVOS dataset and then fine-tuned on the DAVIS dataset. We trained the model with the same configuration similar to CondInst \cite{tian2020conditional} with some changes in hyperparameters as listed below. We define one batch as an iteration.


\subsection{Hyperparameter Optimization} To speed up the process, initially, the network and training parameters were tuned on frame-level evaluation with mAp evaluation metric as used by the COCO data-set. A subset of the training data from YoutubeVOS was used as the validation set. Later on, all the prominent ablation studies were evaluated on the actual validation sets of the DAVIS dataset with $\mathcal{J}$ \& $\mathcal{F}$ Score as the evaluation metric. The tuning procedure was done in a random fashion because of the huge number of parameters available. 

\subsection{YoutubeVOS training:}
We trained our segmentation network on the YoutubeVOS dataset using an SGD optimizer with a gradual warmup till 10000 iterations and batch size of 12. The base learning rate is set to 0.01, and further, it reduces by 0.1 factor after  60000 and 80000 iterations. We train MBVOS till 100K iterations.  We used the ResNet-101 as a backbone feature extractor and ran it on three Quadro RTX 8000 GPU machines.

\subsection{DAVIS Fine-tuning.}
For finetuning on the DAVIS dataset, we set the learning rate very low at 0.001. We evaluate our model after 350 iteration and reported our best model at 6300 iteration. The train time was significantly less becasuse of the small size of this dataset. We trained the models longer but with no improvement in segmentation accuracy. We also trained the model without the pre-trained weights of YoutubeVOS. 


\section{Results} 
We compare our method from two perspectives. The first one is the comparison with our baseline network to demonstrate how motion solely improves the performance. The second one is the comparative evaluation of our method with fully- and self-supervised VOS methods. We use ResNet-101 \cite{he2016deep} backbone for comparison with other state-of-the-art.

\label{sec:result}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{img/sequence5.png}
    \caption{Predictions of our method on DAVIS data-set. Due to semi-supervised evaluation, the first-frame(0th) represents  ground truth annotation mask.}
    \label{fig:video_sequence}\vspace{-1em}
\end{figure}

\subsection{Comparison with Box Supervised Color only Baseline} 
For the sake of comparison, we employ our baseline network and train without motion information. The baseline network's architecture and other parameters remain the same with MBVOS. The generated framewise proposals are tracked similarly to those as mentioned in section \ref{tracking}. Table \ref{tab:davis_sota} and Table \ref{tab:uvos_sota}, demonstrates MBVOS outperform its color only baseline by 3.6\% on DAVIS and 5.3\% on YouTube-VOS dataset. It distinctively shows the superiority of MBVOS and the exploration of motion cues alongside color for VOS.  The advantage of motion supervision is explained in Figure \ref{fig:c_v_m}.
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{img/c_vs_m4.png}
    \caption{A qualitative comparison between baseline(color only) and MBVOS. The baseline model predicts an erroneous mask for the distant man due to color similarity with reflection on the TV case. While the inclusion of motion alleviates this in MBVOS.}
    \label{fig:c_v_m}
\end{figure}


\subsection{Comparison with State-of-the-Art VOS methods}
Table \ref{tab:davis_sota}, shows the performance comparison of MBVOS on DAVIS-2017 validation set.  It depicts MBVOS significantly outperforming the self-supervised benchmark by 7\% $\mathcal{J} \& \mathcal{F}$ score on DAVIS. Furthermore, MBVOS demonstrates superior performance compared to the most fully supervised approaches and achieved a competitive performance with top-performing models. Performance of MBVOS is an indicator that box-guided exploration of simultaneous video cues like motion or color could lead to a potent VOS architecture comparable to fully supervised ones without using ground truth masks. With less expensive box label annotation, we significantly reduce the performance gap with fully-supervised methods that use expensive ground truth mask annotation.  Figure \ref{fig:video_sequence} shows some qualitative examples. We also evaluated our approach on YouTube-VOS \cite{Yang2019} as shown in Table \ref{tab:uvos_sota}. MBVOS achieves 53.5 $\mathcal{J} \& \mathcal{F}$ score, which is better than most self-supervised methods apart from the recently proposed MAST\cite{Lai}, and gives competitive results in comparison with fully supervised methods \cite{osmn,msk,rgmp,onavos}. 

\begin{center}
       \includegraphics[width=\textwidth]{img/teaser.png}
       \captionof{figure}{Qualitative comparison of MBVOS which outperforms self-supervised MAST\cite{Lai} and the fully-supervised FEELVOS\cite{feelvos} and also gives a competitive performance with PReMVOS\cite{premvos} on DAVIS dateset\cite{davis17}. 
    %   Instead of mask supervision, the proposed method uses a pseudo mask generated from color and motion(calculated using a new box guided motion compensation pipeline) to supervise a segmentation network.
       }
       \label{fig:teaser}
    \end{center}

\begin{table}[h]
\centering
% \scriptsize
\begin{tabular}
{cccccc} \toprule
Method & Sup. & $\mathcal{J} \& \mathcal{F}($ Mean $)$ & $\mathcal{J}($ Mean $)$ & $\mathcal{F}($ Mean $)$ \\ \midrule \midrule

Vid. Color.\cite{vid_col}  & Self & $34.0$ & $34.6$ & $32.7$ & \\
CycleTime\cite{cycletime}  & Self & $48.7$ & $46.4$ & $50.0$ & \\
CorrFlow\cite{CorrFlow}  & Self & $50.3$ & $48.4$ & $52.2$ & \\
UVC\cite{uvc} & Self & $59.5$ & $57.7$ & $61.3$ & \\
RPM-Net\cite{rpmnet} & Self & $41.6$ & $41.0$ & $42.2$ & \\
Mug\cite{lu2020learning}  & Self & $56.1$ & $54.0$ & $58.2$ & \\
\textbf{MAST\cite{Lai}} & \textbf{Self} & $\mathbf{65.5}$ & $\mathbf{63.3}$ & $\mathbf{67.6}$ & \\ \midrule

BoxInst$\cite{Tian2020} \dagger$ & Box & $68.9$ & $68.2$ & $69.6$ & \\
\textbf{Ours} & \textbf{Box} & $\mathbf{72.5}$ & $\mathbf{71.5}$ & $\mathbf{73.5}$ \\ \midrule

OSMN\cite{osmn} & Full & $54.8$ & $52.5$ & $57.1$ & \\
OSVOS\cite{osvos}  & Full & $60.3$ & $56.6$ & $63.9$ & \\
SiamMask\cite{siammask} & Full & $56.4$ & $54.3$ & $58.5$ & \\
OSVOS-S\cite{osvos-s}  & Full & $68.0$ & $64.7$ & $71.3$ & \\
GC\cite{gc} & Full & $71.4$ & $69.3$ & $73.5$ & \\
FEELVOS\cite{feelvos} & Full & {$71.5$} & {$69.1$} & {$74.0$} & \\
AFB-URR\cite{afburr} & Full & $74.6$ & $73.0$ & $76.1$ & \\
{PReMVOS\cite{premvos}} & {Full} & {$77.8$} & {$73.9$} & {$81.7$} & \\
CFBI\cite{cfbi} & Full & $81.9$ & $79.1$ & $84.6$ & \\
STM\cite{stm} & Full & $81.8$ & $79.2$ & $84.3$ & \\
\textbf{RMNet\cite{Xie}} & \textbf{Full} & $\mathbf{8 3 . 5}$ & $\mathbf{8 1 . 0}$ & $\mathbf{8 6 . 0}$ & \\ \hline

\end{tabular}
\caption{ State-of-the-art comparison on DAVIS \cite{davis17} validation set. $\dagger$ denotes our baseline method that uses only color.}
\label{tab:davis_sota}
\end{table}




\begin{table}[h]
\centering
% \scriptsize
\begin{tabular}{ccccccc}
\toprule \multirow{2}{*}{ Method } & \multirow{2}{*}{ Sup. } & \multirow{2}{*}{ Overall $\uparrow$} & \multicolumn{2}{c}{ Seen } & \multicolumn{2}{c}{ Unseen } \\
\cline { 4 - 7 } & & & $\mathcal{J} \uparrow$ & $\mathcal{F} \uparrow$ & $\mathcal{J} \uparrow$ & $\mathcal{F} \uparrow$ \\\midrule \midrule
Vid. Color.\cite{vid_col} & Self & $38.9$ & $43.1$ & $38.6$ & $36.6$ & $37.4$ \\
CorrFlow\cite{CorrFlow} & Self & $46.6$ & $50.6$ & $46.6$ & $43.8$ & $45.6$ \\
\textbf{MAST\cite{Lai}} & \textbf{Self} & $\mathbf{6 4 . 2}$ & $\mathbf{6 3 . 9}$ & $\mathbf{6 4 . 9}$ & $\mathbf{6 0 . 3}$ & $\mathbf{6 7 . 7}$ \\ \midrule

BoxInst\cite{Tian2020} $\dagger$ & Box & $48.2$ & $51.6$ & $52.3$ & $44.7.8$ & $44.9$ \\
\textbf{Ours} & \textbf{Box} & $\mathbf{53.5}$ & $\mathbf{58.7}$ & $\mathbf{59.2}$ & $\mathbf{46.3}$ & $\mathbf{48.4}$ \\ \midrule

OSMN\cite{osmn} & Full & $51.2$ & $60.0$ & $60.1$ & $40.6$ & $44.0$ \\
MSK\cite{msk} & Full & $53.1$ & $59.9$ & $59.5$ & $45.0$ & $47.9$ \\
RGMP\cite{rgmp} & Full & $53.8$ & $59.5$ & $-$ & $45.2$ & $-$ \\
OnAVOS\cite{onavos} & Full & $55.2$ & $60.1$ & $62.7$ & $46.6$ & $51.4$ \\
RVOS\cite{rvos} & Full & $56.8$ & $63.6$ & $67.2$ & $45.5$ & $51.0$ \\
OSVOS\cite{osvos} & Full & $58.8$ & $59.8$ & $60.5$ & $54.2$ & $60.7$ \\
S2S\cite{s2s} & Full & $64.4$ & $71.0$ & $70.0$ & $55.5$ & $61.2$ \\
{PReMVOS\cite{premvos}} & {Full} & {$66.9$} & {$71.4$} & {$75.9$} & {$56.5$} & {$63.7$} \\
STM\cite{stm} & Full & $79.4$ & $79.7$ & $84.2$ & $72.8$ & $80.9$ \\
\textbf{RMNet\cite{Xie}} & \textbf{Full} & $\mathbf{81.5}$ & $\mathbf{82.1}$ & $\mathbf{85.7}$ & $\mathbf{75.7}$ & $\mathbf{82.4}$ \\ \hline
\end{tabular}
\caption{ State-of-the-art comparison on Youtube-VOS\cite{yvos2018}. 
$\dagger$ denotes our baseline method that uses only color.}
\label{tab:uvos_sota}
\end{table}


\pagebreak

\section{Limitations and further scope of improvement}
Compared to DAVIS (in Table \ref{tab:davis_sota}), performance of MBVOS deteriorated for YouTube VOS (in Table \ref{tab:uvos_sota}). We observe that there are two primary reasons which lead to a decline in performance. First, the object re-identification network \cite{li2017video} from PReMVOS \cite{premvos} we used as part of our tracking pipeline is trained on DAVIS. Hence, most of the scenarios where objects undergo a change in appearance in the next consecutive frames have failed to re-identify the proposals from the previous frame. Second, video sequences from YouTube-VOS are relatively long compared to DAVIS and suffer more occlusions. 
\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{img/limitation2.png}
    \caption{An example of negative scenario: tracking failure in YouTube VOS. The fish is present in our segmentation proposal but the tracker could not track it after it was occluded.}
    \label{fig:limitation}
\end{figure}
Figure \ref{fig:limitation} shows the initial appearance of fish, its occlusion, and its re-appearance from occlusion alongside our segmentation proposal and tracker prediction. We can observe that despite having the proposal after the fish appeared from occlusion, the tracker failed to track the fish with the re-identification score and simple bipartite matching. This limitation can be addressed in two ways. First, the re-identification network can be fine-tuned with YouTube-VOS, which will help to re-identify objects in consecutive frames. Second, state-of-the-art tracking such as \cite{Xie} can be employed with a more extended temporal matching scheme that can effectively track the occluded object and effectively re-identify them even after the occlusion. Due to the scope of this work on box-supervised VOS, we will address these issues in our future work. 

\pagebreak
\section{Ablation Studies}
We investigate four primary aspects of our method: improvement due to motion, motion pipeline and affinity loss, pre-training, and finally, experimenting with predicted foreground pixels. Unless otherwise specified, the ablation study has been conducted using ResNet-50\cite{he2016deep} as the backbone and trained with the DAVIS training dataset for faster computation.

\subsection{Motion} Table \ref{tab:ablation_motion}, shows the influence of different motion filters and their combination as discussed in Sec. \ref{sec:motion_calc}. Unfiltered motion is inherently noisy and hurts the performance, whereas adding more filters for refinement of motion improves the performance. Starting from the box filter (BF) to the three-frame filter (3F)  has incrementally refined motion and improved the segmentation performance. \\
Table \ref{tab:ablation_fusion}, describes the impact of the combination of color and motion during supervision as stated in Sec. \ref{sec:loss}. Here, the third row is the intersection affinity as in Eq. \ref{eq:aff_i} which is replaced with a union operation in the first row's experiment. Taking the union of color and motion supervision performed worse than when motion was used alone. However, the intersection of motion and color similarity gives the best performance in comparison to the union, hence it bolsters our strategy on generating small number of yet high precision foreground pixels. 
\subsection{Backbone and pre-training} Finally, Table \ref{tab:ablation_backbone}, depicts the type of input backbone and data-sets used during training. A larger backbone network and pre-training help learn more expressive features and improve performance. 

\begin{table*}
\centering
\begin{tabular}[t]{c|c}\toprule
Filters & $\mathcal{J}\& \mathcal{F}($Mean$)$ \\\midrule\midrule
None  & 68.5 \\
% FBF & & 70.7\\
% 3F  & &70.9 \\
BF*  &69.1 \\
BF* + 3F& 69.2 \\
% 3F + FBF  & 71.7 \\
BF* + FBF + 3F &  70.5 \\
% \textbf{BF* + FBF + 3F}  & \textbf{Resnet-101} &  \textbf{72.5} \\
\bottomrule
\end{tabular}
    \begin{tablenotes}
    \centering
        \smaller
        \item BF*: Box Filter, FBF: Forward-Backward Filter, 3F: 3-Frame Difference
    \end{tablenotes}
\caption{\centering Impact of the proposed filters and their combination for motion refinement and improvement.}
\label{tab:ablation_motion} 
\end{table*}


\begin{table*}
\centering
\begin{tabular}[t]{c|c}\toprule
Supervision  & $\mathcal{J}\& \mathcal{F}($Mean$)$ \\\midrule\midrule
Motion Only  &  69.4 \\
Color $\cup$ Motion  & 68.8\\
Color $\cap$ Motion  &  70.5 \\
\bottomrule
\end{tabular}
\caption{\centering Effect of combined motion and color utilization on pseudo mask generation.}
\label{tab:ablation_fusion} 
\end{table*}


\begin{table*}
\centering
\begin{tabular}[t]{c|c|c}\toprule
Backbone & Train Data & $ \mathcal{J}\& \mathcal{F}($Mean$)$ \\\midrule\midrule
ResNet-50 & D & 70.5\\
ResNet-50 & DY &  72.1 \\
\textbf{ResNet-101} & \textbf{DY} &  \textbf{72.5}\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\centering
    \smaller
    \item 
       D: DAVIS, Y: YVOS, 
\end{tablenotes}
\caption{\centering Effect of various backbone networks and pre-training.}
\label{tab:ablation_backbone}
\end{table*}





\subsection{Optical Flow Calculation}
Optical flow calculates a pixel's relative position change from one frame to the next. It can be classified into sparse and dense versions. The former calculates flow for a subset, whereas the latter for all pixels in a given image. Therefore, sparse optical flow is faster. Three optical flow implementations were tested in the motion calculation pipeline and the results are reported in table \ref{tab:opt-flow} with $\tau_M$ = 0.75 and $\tau_C$ =0.1. The sparse optical flow \cite{bouguet2001pyramidal} gave the best result. So extra computation power for generating dense optical flow with Farneback\cite{Farneback}, or PerceiverIO\cite{Jaegle} is not necessary for performance. 

\begin{table}[!htp]\centering
% \scriptsize
\begin{tabular}{c|c}\toprule
Optical Flow & $\mathcal{J}\& \mathcal{F}($Mean$)$ \\\midrule \midrule
Sparse &\textbf{70.5}\\
Fernaback &65.4 \\
PerceiverIO &67.6 \\
None & 68.9 \\
\bottomrule
\end{tabular}
\caption{Optical Flow Calculation on  YVIS-train-val}
\label{tab:opt-flow}
\end{table}


\subsection{Color and Motion Similarity Threshold} We investigate the role of similarity score for both color and motion. A similarity threshold dictates how similar two-pixel have to be assigned in the same class. We employed a random search to find the appropriate similarity for combined color and motion properties.% is required in the absence of an analytical formulation. 
Table \ref{tab:hpo_sim_thr}, shows the performance of our model on multiple similarity threshold. A notable characteristic can be observed, higher-value leads to better results especially for motion. A low value would allow more pairs to be classified as the same class, known as positive pairs, with a significant loss of precision. On the other hand, a high value would generate fewer positive pairs but with high precision. The higher threshold value of motion endorses that motion is comparatively noisy and only high confidence motion generates positive pairs.  

The best result came with a high similarity threshold for motion. In most cases, a significant portion of an object moves with similar velocity but can have slightly varying colors. Best performance with the higher motion threshold reflects this scenario. This experiment was done with an additional median filter at the end of motion calculation, so the results are slightly better than other ablation studies.



\begin{table}[!htp]\centering
% \scriptsize
\begin{tabular}{c|c|c}\toprule
$\tau_M$ & $\tau_C$ & $\mathcal{J}\& \mathcal{F}($Mean$)$\\\midrule\midrule
0.1 &0.1 & 69.1\\
0.001 &0.1 & 69.1\\
0.95 &0.1 & 69.5\\
0.1 &0.3 & 68.9 \\
\textbf{0.75} & \textbf{0.1} & \textbf{70.5} \\
0.9 &0.1 & 69.1\\
0.001 &0.3 & 68.9\\
0.3 &0.1 & 69.1 \\
% 0.95 &0.3 &24.33 \\
0.3 &0.3 & 68.8\\
0.75 &0.3 & 68.9\\
\bottomrule
\end{tabular}
\caption{\centering Optimal color and motion similarity threshold search on DAVIS trained with ResNet-50 backbone and without Youtube-VOS pretraining weights.}
\label{tab:hpo_sim_thr}
\end{table}

\subsection{Predicted Foreground pixels } Table \ref{tab:ablation-gt} shows a proof-of-concept for the inclusion of a filter-based motion pipeline and its contribution to generating high-precision pixels. To calculate metrics (i.e., true positives) related to F1 score, precision, and recall, ground truth segmentation masks were used here. However, ground truth masks have never been used in training or performing filter optimization. Pixels greater than the threshold value of 0.5 are labeled as foreground, with the motion being normalized between 0 and 1. 
\begin{table*}[!htp]\centering
% \scriptsize
\begin{tabular}{c|c|c|c|c}
\toprule
{Filters} & {F1} & {Precision} & {Recall} & {Avg. FPS}\\
\midrule \midrule
None & 0.404 & 0.318 & 0.553 & \textbf{9.99}\\
BF* & \textbf{0.482} & 0.397 & \textbf{0.612} & 4.05 \\
FBF & 0.425 & 0.346 & 0.550 & 9.37 \\
3F & 0.399 & 0.359 & 0.449 & 4.94 \\
BF + FBF & 0.481 & 0.397 & 0.611 & 3.93\\
BF + 3F & 0.462 & \textbf{0.422} & 0.509 & 2.07\\
FBF + 3F & 0.402 & 0.364 & 0.448 & 4.70\\
BF* + 3F + FBF & 0.460 & \textbf{0.421} & 0.507 & 1.96\\

\bottomrule
\end{tabular}
    \begin{tablenotes}
        \smaller
        \item 
        \begin{center}
            BF*: Box Filter, FBF: Forward-Backward Filter, 3F: 3-Frame Difference, FPS: Frame per second
        \end{center}
    \end{tablenotes}
\caption{ The capability of different filter combinations to extract foreground pixels for DAVIS trainval data-set.}
\label{tab:ablation-gt}
\end{table*}
It can be observed from Table \ref{tab:ablation-gt} that using raw motion results in low precision, which is a deteriorating factor for our method. On the contrary, refined motion increases precision, resulting in improved quality of supervision and performance.

% \section{Evaluation Metric}

% \section{Data Related}
% \subsection{Removing still objects}
% Toilet, Bucket, Sign, Others
% \subsection{Apply on other data set like DAVIS??}

% \section{Network Related}
% \begin{itemize}
%     \item Resnet-50 (Done)
%     \item Resnet-101 (Running)
%     \item Others
% \end{itemize}

% \section{Optimization}
% \begin{itemize}
%     \item Batch size (16 running)
%     \item Scheduled time
%     \item Others
% \end{itemize}

% \section{Loss Related}
% \begin{itemize}
%     \item Union(Running)
%     \item Intersection(Done)
%     \item Motion only(Running)
%     \item Normalized Channel(Running)
% \end{itemize}

% \section{Level of Supervision}
% \begin{itemize}
%     \item No Motion or Color
%     \item Only Color(Done)
%     \item Only Motion (Running)
%     \item Motion + Color (Done)
%     \item Motion + Channel (Done)
%     \item Fully Supervised
% \end{itemize}


% \section{Motion Compensation}
% \begin{itemize}
%     \item box filter
%     \item three frame filter
%     \item forward backward filter
% \end{itemize}

% \section{Motion Calculation}
% \begin{itemize}
%     \item sparse opt flow (Done)
%     \item fernaback opt flow (Done)
%     \item perceiverIO (Running)
% \end{itemize}

% \section{Previous Work}
% \begin{itemize}
%     \item Boxinst (Done)
%     \item BBMA 
%     \item Background-Aware Pooling and
% \end{itemize}

==> Master's Thesis Report/07-Conclusion.tex <==
\chapter{Conclusion}
In this work, we have shown the potential of MBVOS, the first motion-aware, box-supervised video segmentation network. Furthermore, we have demonstrated that exploring video cues in a weakly supervised setup could lead to a competitive VOS framework. The core idea of MBVOS is to refine and leverage motion, subsequently, combine it with color channels if both share similar characteristics. Our proposed method significantly reduces the performance gap with top-performing fully supervised methods on the DAVIS dataset. At the same time, we are addressing some of the complex scenarios in VOS, such as the camouflage effect. We will develop a more accurate motion compensation pipeline and extended temporal proposal tracking for an efficient VOS framework for future work. 

==> Master's Thesis Report/intro_old.tex <==
\chapter{Ein Kapitel}

Das ist die Ebene {\tt chapter}.

\section{Ein Abschnitt}

Das ist die Ebene {\tt section}.

\subsection{Ein Unterabschnitt}

Das ist die Ebene {\tt subsection}.

\subsubsection{Ein Unterunterabschnitt}
\label{sec:a}

Das ist die Ebene {\tt subsubsection}.

\subsubsection{Noch ein Unterunterabschnitt}
\label{sec:b}

Wer \ref{sec:a} sagt, mu"s auch \ref{sec:b} sagen.

\subsection{Noch ein Unterabschnitt}

Das ist ein gew"ohnlicher Absatz.

\paragraph{Ein Absatz mit Titel}

Das ist die Ebene {\tt paragraph}.

\subparagraph{Ein Unterabsatz mit Titel}

Das ist die Ebene {\tt subparagraph}.

\subsection*{Ein nicht numerierter Unterabschnitt}

Dieser Unterabscnitt erscheint nicht im Inhaltsverzeichnis.

\section{Beispiele}
Dieses Beispieldokument wurde mit dem \LaTeX-Paket {\tt dbstmpl.sty} erzeugt.
{\tt dbstmpl.sty} definiert Befehle zum Erzeugen von einigen
h"aufig gebrauchten Symbolen.

\begin{align}
  \N \subset \Z \subset \Q \subset \R \subset \C
\end{align}

Weitere Symbole k\"onnen im {\tt symbols-a4.pdf}-Dokument, das f\"ur
gew\"ohnlich bei \LaTeX-Distributionen mitgeliefert wird, nachgeschlagen
werden. Alternativ gibt es diverse Hilfeseiten im Netz.

Au"serdem werden automatisch einige zus"atzliche Pakete geladen.
Mit dem Paket {\tt graphicx} k"onnen Grafiken eingebunden werden.
Abbildung~\ref{fig:dbslogo} zeigt das Logo der LFE f"ur Datenbanksysteme.

\begin{figure}
  \begin{center}
    \includegraphics[width=2cm]{logo-dbs.png}
  \end{center}
  \caption{Altes Logo der LFE f"ur Datenbanksysteme.
    \label{fig:dbslogo} % Figures und Tables können gelabelt werden.
    % Es empfiehlt sich, dies in der Caption zu machen
  }
\end{figure}

{\tt amsmath} erlaubt die bequeme Alignierung von mehrzeiligen Formeln:

\begin{align}
  f(a,b) &= (a-b)^2 \label{eq:aMinusbSq}\\
    &= a^2 - 2 a b + b^2 \label{eq:aMinusbSqResolved}
\end{align}

Zus\"atzlich k\"onnen diese Formeln auch referenziert werden. In~\eqref{eq:aMinusbSq}
wird das Problem gestellt und in~\eqref{eq:aMinusbSqResolved} wird es etwas
aufgel\"ost. Nat\"urlich k\"onnen die Gleichungen auch ohne Klammern
referenziert werden: \ref{eq:aMinusbSq}, \ref{eq:aMinusbSqResolved}.

Das in diesem Dokument geladene Paket {\tt subfigure} (oben eingebunden durch
\verb=\usepackage{subfigure}=) erlaubt das Erzeugen von Unterabbildungen.
Abbildung~\ref{fig:logos} enth"alt zwei Unterabbildungen.
Abbildung~\ref{fig:logos-a} zeigt nochmal das Logo der LFE f"ur
Datenbanksysteme, \ref{fig:logos-b} zeigt das Logo der
Ludwig-Maximilians-Universit"at.

\begin{figure}
  \begin{center}
    \subfigure[Altes DBS-Logo.\label{fig:logos-a}]{
      \makebox[0.48\textwidth]{
        \includegraphics[width=2cm]{logo-dbs.png}}}
    \hspace{\fill}
    \subfigure[Uraltes LMU-Logo.\label{fig:logos-b}]{
      \makebox[0.48\textwidth]{
        \includegraphics[width=5cm]{logo-lmu.png}}}
  \end{center}
  \caption{Zwei Logos.}
  \label{fig:logos}
\end{figure}

Tabelle~\ref{tab:quadratzahlen} zeigt die ersten f"unf Quadratzahlen.

\begin{table}
  \begin{center}
  \begin{tabular}{|r|r|}
    \hline \makebox[1cm]{$x$} & \makebox[1cm]{$x^2$}\\
    \hline\hline 1 &  1\\
    \hline 2 &  4\\
    \hline 3 &  9\\
    \hline 4 & 16\\
    \hline 5 & 25\\
    \hline
  \end{tabular}
  \end{center}
  \caption{Die Zahlen 1 bis 5 und ihre Quadrate.}
  \label{tab:quadratzahlen}
\end{table}

Folgenderma\ss en wird Literatur referenziert.
DBSCAN~\cite{EKSX96} und OPTICS~\cite{ABKS99} sind Beispiele f\"ur
dichtebasierte Clusteringverfahren. Diese Eintr\"age werden als
{\tt bibitem} im {\tt .bbl}-File referenziert. Um dieses File braucht man
sich erfreulicherweise nicht zu k\"ummern, weil es automatisch aus einer
Sammlung von BibTeX-Eintr\"agen in einem Literatur-File gebildet werden
kann. Hier ist wichtig, dass dieses File den BibTeX-Konventionen
\footnote{{\tt http://www.tex.ac.uk/tex-archive/biblio/bibtex/contrib/doc/btxdoc.pdf}}
entspricht, sonst kommen kreative Fehlermeldungen. Daf\"ur braucht es
besagte Literatur-Sammlung -- hier {\tt dbstmpl.bib}
und einen Literatur-Stil, den man auch selber definieren kann, wie
etwa {\tt dbstmpl.bst}.

\section{Bemerkungen}

Eine "Ubersicht "uber alle Abbildungen und Tabellen einer Arbeit
verschaffen das Abbildungs- und das Tabellenverzeichnis. Diese
sollten entweder nach dem Inhaltsverzeichnis oder (wie in diesem
Dokument) vor dem Literaturverzeichnis eingef"ugt werden.
Je nach Bedarf und Umfang der Arbeit k"onnen auch Verzeichnisse
f"ur Definitionen, S"atze oder Lemmata angelegt oder nicht
ben"otigte Verzeichnisse weggelassen werden.

\appendix

\chapter{Ein Anhang}

Im Anhang kann auf Implementierungsaspekte wie Datenbankschemata
oder Programmcode eingegangen werden.

\section{\protect{pdflatex} vs.\ \protect{latex}}

Dieses Dokument wird mit {\tt pdflatex} gebaut. Das ist n\"otig, wenn
wie hier Bilder im {\tt .jpg}, {\tt .png} oder {\tt .pdf}-Format eingebunden
werden. Alternativ kann auch alles \"uber das klassische \LaTeX-Kommando
laufen: \verb=latex dbsba=. Damit wird ein {\tt .dvi} erstellt, welches
erst mit {\tt dvipdf} zu {\tt .pdf} konvertiert werden muss. Dies
bedeutet, dass Bilder nur noch als {\tt .eps} eingebunden werden
k\"onnen. {\em Merke: {\tt .pdf}-affine und {\tt .eps}-Bilder k\"onnen
NICHT kombiniert werden, also entweder oder.}

\section{Ich will aber englisch!}

Ihr d\"urft auch gerne englische \the\arbeit en schreiben. Daf\"ur m\"usst
ihr im Stylefile {\tt dbstmpl.sty} die Zeile
\verb=\RequirePackage[english,german]{babel}= durch
\verb=\RequirePackage[german,english]{babel}= austauschen. Dann hei\ss en
Chapter wieder Chapter und nicht Kapitel, etc.

\section{Ich h\"atte da einen eigenen Stil.}

Ihr k\"onnt auch eigene Stile definieren und verwenden, wenn er die
Informationen des Deckblatts und die darauffolgende Erkl\"arung
enth\"alt, sowie die Gnade des Betreuers gefunden hat (es
empfiehlt sich also, fr\"uhzeitg kurz nachzufragen).

\section{Hilfe?}

Gibt es online zuhauf:

\begin{description}
  \item[Das \LaTeX Kochbuch]~\\{\tt http://www.uni-giessen.de/hrz/tex/cookbook/cookbook.html}
  \item[CTAN] {\tt http://www.ctan.org/} zum manuellen Download von Stylefiles
      und deren Dokumentation
  \item[Diverse Mathe-Tweaks]~\\ \verb=http://meta.wikimedia.org/wiki/Help:Displaying_a_formula=
  \item[B\"uchersuche mit BibTeX -Unterst\"utzung] {\tt http://lead.to/amazon/en/}
  \item[JabRef] Java-basierter BibTeX -Manager {\tt http://jabref.sourceforge.net/}
  \item[FAQs] {\tt http://www.tex.ac.uk/cgi-bin/texfaq2html}
\end{description}

Und zur Not versteht auch euer Betreuer vermutlich was davon.

==> result_temp.tex <==
% We may remove YVIS train-test after we get tracking result
\begin{table*}[!t]\centering
\caption{Comparison with state-of-the-art (mAp).}
\scriptsize
\begin{tabular}{c|c|c|c|c}\toprule
Supervision&Method & Coco test-dev & YVIS-train-test &  DAVIS-val \\\midrule \midrule
\multirow{8}{*}{Mask} 
&CondInst(R-50) &37.8 &\textit{30} &\textit{20.42} \\
&VisTR(R-50)\cite{Wangvistr} & - &36.2 & - \\
&MaskProp(R-50)\cite{Bertasius2019} & - &40.0 & - \\
&IFC(R-50)\cite{Hwang} & - &\textbf{42.8} & - \\
\cmidrule{2-5}
&CondInst(R-101) &39.1 &{32.72} & {Training} \\
&VisTR(R-101)\cite{Wangvistr} & - & 40.1 & - \\ 
&MaskProp(R-101)\cite{Bertasius2019} & - & 42.5 & - \\
&IFC(R-101)\cite{Hwang} & - & \textbf{44.6} & - \\ 
\midrule

\multirow{9}{*}{Box}
&DiscoBox(R-50) & {32} & - & - \\
&BoxInst(R-50) &\textbf{32.1} & $23.67^{[a]}$ $\pm$ 0.5 &\textit{12.76}\\
&\textbf{Ours(R-50)}$^{[b]}$ &- &\textbf{24.84$^{[a]}$} $\pm$ 0.4 &\textbf{\textit{14.32}}\\
\cmidrule{2-5}
&BBAM(R-101) & {25.7} & - & -\\
&BoxInst(R-101) &\textbf{33.2} &25.44 &{Training}  \\
&\textbf{Ours(R-101)} &- &\textbf{26.28} &{Training}  \\
\cmidrule{2-5}
&BoxInst(R-101-DCN) &35 &Training &Training  \\
&{DiscoBox(R-101-DCN)} &{\textbf{35.8}} & - & - \\
&\textbf{Ours(R-101-DCN)} &- &{Training}  &{Training}  \\
% \midrule
% Label &Temp. Mask &- &$14.1^[c]$ &- \\
\bottomrule
\end{tabular}
    \begin{tablenotes}
        \smaller
        \item \begin{center}
                [a] Trained 5 times and average result reported. [b] Without percentile filter
                % [c]Result with a publicly unavailable split reported in their paper.
              \end{center}
    \end{tablenotes}
    \label{tab:sota}
\end{table*}


\begin{table*}[!htp]\centering
\scriptsize
\begin{tabular}
{ccccccccc}
\hline Method  & Backbone & Training Data & Supervision & $\mathcal{J} \& \mathcal{F}($ Mean $)$ & $\mathcal{J}($ Mean $)$ & $\mathcal{F}($ Mean $)$ & $\mathcal{J}($ Recall $)$ & $\mathcal{F}($ Recall $)$ \\
\hline Vid. Color.  & ResNet-18  & $\mathrm{K}$ & Self & $34.0$ & $34.6$ & $32.7$ & $X$ & $X$\\
CycleTime  & ResNet-50 & $\mathrm{V}$ & Self & $48.7$ & $46.4$ & $50.0$ & $X$ & $X$\\
CorrFlow  & ResNet-18  & $\mathrm{O}$ & Self & $50.3$ & $48.4$ & $52.2$ & $X$ & $X$\\
UVC  & ResNet-18 & $\mathrm{K}$ & Self & $59.5$ & $57.7$ & $61.3$ & $X$ & $X$\\
RPM-Net & ResNet-101 & DY & Self & $41.6$ & $41.0$ & $42.2$ & $X$ & $X$\\
Mug & ResNet-50 & O & Self & $56.1$ & $54.0$ & $58.2$ & $X$ & $X$\\
MAST & ResNet-18  & Y & Self & $65.5$ & $63.3$ & $67.6$ & $X$ & $X$\\
\hline OSMN & VGG-16 & ICD & Full & $54.8$ & $52.5$ & $57.1$ & $X$ & $X$\\
SiamMask & ResNet-50  & ICY & Full & $56.4$ & $54.3$ & $58.5$ & $X$ & $X$\\
OSVOS & VGG-16 & ID & Full & $60.3$ & $56.6$ & $63.9$ & $X$ & $X$\\
OSVOS-S & VGG-16 & IPD & Full & $68.0$ & $64.7$ & $71.3$ & $X$ & $X$\\
GC & ResNet-50 & ISEHD & Full & $71.4$ & $69.3$ & $73.5$ & $X$ & $X$\\
FEELVOS & Xception-65 & ICDY & Full & $71.5$ & $69.1$ & $74.0$ & $X$ & $X$\\
\hline Ours & ResNet-50 & DY & Box & $\mathbf{72.2}$ & $\mathbf{X}$ & $\mathbf{X}$ & $\mathbf{X}$ & $\mathbf{X}$\\
Ours & ResNet-101 & DY & Box & $\mathbf{72.8}$ & $\mathbf{X}$ & $\mathbf{X}$ & $\mathbf{X}$ & $\mathbf{X}$\\
Ours & ResNet-101-DCN & DY & Box & $\mathbf{73}$ & $\mathbf{X}$ & $\mathbf{X}$ & $\mathbf{X}$ & $\mathbf{X}$\\
\hline AFB-URR & ResNet-50 & ICPSED & Full & $74.6$ & $73.0$ & $76.1$ & $X$ & $X$\\
CFBI & ResNet-101 & ICDY & Full & $81.9$ & $79.1$ & $84.6$ & $X$ & $X$\\
STM & ResNet-50 & ICPSEDY & Full & $81.8$ & $79.2$ & $84.3$ & $X$ & $X$\\
RMNet & ResNet-50 & ICPSEDY & Full & $\mathbf{8 3 . 5}$ & $\mathbf{8 1 . 0}$ & $\mathbf{8 6 . 0}$ & $X$ & $X$\\
\hline
\end{tabular}
\caption{State of the art comparison on DAVIS-2017 validation set. Training Data symbols: C=COCO, D=DAVIS, E=ECSSD, H=HKU-IS, I=ImageNet, K=Kinetics, M=Mapillary, O=OxUvA, P=PASCAL-VOC, S=MSRA10K, V=VLOG, Y=YouTube-VOS.}
\end{table*}
